Rate-Independent Gradient Crystal Plasticity Theory -- Robust Algorithmic Formulations based on Incremental Energy Minimization

Numerically robust algorithmic formulations suitable for rate-independent crystal plasticity are presented. They cover classic local models as well as gradient-enhanced theories in which the gradients of the plastic slips are incorporated by means of the micromorphic approach. The elaborated algorithmic formulations rely on the underlying variational structure of (associative) crystal plasticity. To be more precise and in line with so-called variational constitutive updates or incremental energy minimization principles, an incrementally defined energy derived from the underlying time-continuous constitutive model represents the starting point of the novel numerically robust algorithmic formulations. This incrementally defined potential allows to compute all variables jointly as minimizers of this energy. While such discrete variational constitutive updates are not new in general, they are considered here in order to employ powerful techniques from non-linear constrained optimization theory in order to compute robustly the aforementioned minimizers. The analyzed prototype models are based on (1) nonlinear complementarity problem (NCP) functions as well as on (2) the augmented Lagrangian formulation. Numerical experiments show the numerical robustness of the resulting algorithmic formulations. Furthermore, it is shown that the novel algorithmic ideas can also be integrated into classic, non-variational, return-mapping schemes.

==> commands.tex <==
% Definitions file
% for macros, operators, ...

% Remark
\newtheorem{remark}{Remark}

% some coloring
\newcommand{\red}[1]{{\color{red} #1}}

% some new commands
\newcommand{\lengthscale}{l_\mathrm{e}}
\newcommand{\X}{\boldsymbol{X}}
\newcommand{\x}{\boldsymbol{x}}
\renewcommand{\d}{\ensuremath{\mathrm{d}}}
\newcommand{\timeinterval}{\mathbb{T}}
\newcommand{\npi}{\ensuremath{{n+1}}}
\newcommand{\nmi}{\ensuremath{{n-1}}}
\newcommand{\Pintr}{\ensuremath{P^\mathrm{intr}}}
\newcommand{\Ploc}{\ensuremath{P^\mathrm{loc}}}
\newcommand{\Pglob}{\ensuremath{P^\mathrm{glob}}}

\newcommand{\resl}{\boldsymbol{R}^\mathrm{l}}
\newcommand{\resg}{\boldsymbol{R}^\mathrm{g}}
\newcommand{\Hessl}{\boldsymbol{h}^\mathrm{l}}
\newcommand{\Hessg}{\boldsymbol{h}^\mathrm{g}}
\newcommand{\Gradl}{\boldsymbol{g}^\mathrm{l}}
\newcommand{\Gradg}{\boldsymbol{g}^\mathrm{g}}

\newcommand{\boldalpha}{\boldsymbol{\alpha}}
\newcommand{\boldQ}{\boldsymbol{Q}}

\newcommand{\dofsetg}{\boldsymbol{\mathcal{Z}}^{\mathrm{g}}}
\newcommand{\dofsetl}{\boldsymbol{\mathcal{Z}}^{\mathrm{l}}}
\newcommand{\dofvecg}{\boldsymbol{{Z}}^{\mathrm{g}}}
\newcommand{\dofvecl}{\boldsymbol{{Z}}^{\mathrm{l}}}
\newcommand{\pdir}{\boldsymbol{{Z}}^{\mathrm{dir}}}

\newcommand{\frstderiv}{\frac{\partial g(\vec{x})}{\partial \vec{x}}}
\newcommand{\scndderiv}{\frac{\partial^2 g(\vec{x})}{\partial \vec{x}^2}}
\newcommand{\Hessian}{\ensuremath{\mathbf{H}}}
\newcommand{\Gradient}{\ensuremath{\mathbf{G}}}
\newcommand{\hessian}{\ensuremath{H}}
\newcommand{\gradient}{\ensuremath{G}}

\newcommand{\refconf}{\mathcal{B}_0}
\newcommand{\defconf}{\mathcal{B}_\mathrm{t}}

\newcommand{\defmap}{\boldsymbol{\varphi}}
\newcommand{\Pstress}{\boldsymbol{P}}
\newcommand{\bodyforce}{\boldsymbol{B}}
\newcommand{\Diss}{\mathcal{D}}
\newcommand{\var}{\delta}

\newcommand{\Qi}{{Q_\mathrm{i}}}
\newcommand{\Qitilde}{{\tilde{Q}_\mathrm{i}}}
\newcommand{\Qzero}{{Q_0}}
\newcommand{\Qzerotilde}{{\tilde{Q}_0}}
\newcommand{\Qinf}{Q_\infty}

\newcommand{\bodyref}{{\mathcal{B}_0}}
\newcommand{\bodycur}{{\mathcal{B}_\mathrm{t}}}
\newcommand{\Lp}{{\boldsymbol{L}^\mathrm{p}}}
\newcommand{\intfac}{f}
\newcommand{\intfacapprox}{\hat{\intfac}}
\newcommand{\Je}{{J^\mathrm{e}}}
\newcommand{\Jp}{{J^\mathrm{p}}}

\newcommand{\Ce}{{\boldsymbol{C}^\mathrm{e}}}
\newcommand{\Cedev}{\bar{\boldsymbol{C}}^\mathrm{e}}
\newcommand{\F}{\boldsymbol{F}}
\newcommand{\Fe}{{\F^\mathrm{e}}}
\newcommand{\Fedev}{{\bar{\F}^\mathrm{e}}}

\newcommand{\Fp}{{\ensuremath{\F^\mathrm{p}}}}
\newcommand{\Etensor}{\mathsf{\boldsymbol{E}}}
\newcommand{\Sig}{{\boldsymbol{\Sigma}}}
\newcommand{\unity}{\boldsymbol{1}}

\newcommand{\disp}{\boldsymbol{\varphi}}
\newcommand{\phip}{\varphi_\mathrm{p}}
\newcommand{\Thetaeq}{\tilde{\Theta}}
\newcommand{\Ptemp}{\mathcal{P}_\Theta}
\newcommand{\Pdisp}{\mathcal{P}_{\disp}}
\newcommand{\extforce}{{\boldsymbol{f}^\mathrm{ext}}}

\newcommand{\Dint}{\mathcal{D}_{\mathrm{int}}}
\newcommand{\hflux}{\boldsymbol{H}}
\newcommand{\hsource}{H_0}
\newcommand{\eflux}{\boldsymbol{S}}
\newcommand{\esource}{S_0}
\newcommand{\tempgrad}{\ensuremath{{\boldsymbol{G}}}}
%\newcommand{\isopot}{\mathcal{I}_\mathrm{inc}^\mathrm{iso}}
%\newcommand{\isopotred}{\mathcal{I}_\mathrm{inc}^\mathrm{iso,red}}

\newcommand{\isopotrate}{\dot{\mathcal{I}}_\mathrm{inc}^\mathrm{iso}}
\newcommand{\pot}{\mathcal{I}_{\mathrm{inc}}}
\newcommand{\potred}{\mathcal{I}_\mathrm{inc}^\mathrm{red}}
\newcommand{\potrate}{\dot{\mathcal{I}}_{\mathrm{inc}}}
\newcommand{\dlambda}{\Delta \lambda}

\newcommand{\fhat}{\hat{f}}
\newcommand{\flowdir}{\boldsymbol{M}}
\newcommand{\boldzero}{\boldsymbol{0}}
\newcommand{\dofs}{\boldsymbol{\mathcal{Z}}}

\newcommand{\alphai}{\alpha_\mathrm{i}}
\newcommand{\omegah}{\omega_\mathrm{h}}
\newcommand{\omegay}{\omega_\mathrm{y}}
\newcommand{\Hi}{H_\mathrm{i}}

% spaces
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Duals}{\mathbb{D}}
\newcommand{\Complexs}{\mathbb{C}}

% some other macros
\newcommand{\norm}[1]{\| {#1} \|}
\newcommand{\integral}[4]{\int \limits_{#1}^{#2} {#3} \, \mathrm{d} {#4} }
\newcommand{\EXP}[1]{\mathrm{EXP} \left({#1} \right)}
\newcommand{\pdiff}[2]{\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\diff}[2]{\frac{\mathrm{d} {#1}}{\mathrm{d} #2}}
\newcommand{\variation}[2]{\delta_{#2} {#1}}
\newcommand{\transposed}[1]{\ensuremath{{#1}^\mathrm{T}}}
\newcommand{\transinv}[1]{\ensuremath{{#1}^\mathrm{-T}}}

\newcommand{\eye}{\unity}
\newcommand{\Isym}{\boldsymbol{\mathrm{I}}^{4}_{\mathrm{sym}}}
\newcommand{\Isymdev}{\boldsymbol{\mathrm{I}}^{4}_{\mathrm{sym,dev}}}

% notation
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\dual}[1]{\underline{#1}}

% new operators
\DeclareMathOperator{\dev}{dev}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\zh}{z_\mathrm{h}}
\DeclareMathOperator{\zQi}{\zh}
\DeclareMathOperator{\zy}{z_\mathrm{y}}
\DeclareMathOperator{\zQzero}{\zy}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\DUALa}{\mathfrak{D}_1}
\DeclareMathOperator{\DUALb}{\mathfrak{D}_2}
\DeclareMathOperator{\DUALab}{\mathfrak{D}_{12}}
\DeclareMathOperator*{\stat}{stat}
\DeclareMathOperator{\Sigeq}{\Sigma^\mathrm{eq}}
\let\Re\relax
\DeclareMathOperator{\Re}{\mathfrak{R}}

%\DeclareMathOperator{\div}{div}
%\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Div}{Div}
\DeclareMathOperator{\Grad}{Grad}
\DeclareMathOperator{\DIV}{DIV}
\DeclareMathOperator{\GRAD}{GRAD}
\DeclareMathOperator{\Assembling}{Assembling}
% Assembly Operator
%\usepackage{relsize}
%\DeclareMathOperator*{\A}{ \underset{e}{\mathlarger{\mathlarger{\mathlarger{\boldsymbol{\mathsf{A}}}}} }}

==> definitions.tex <==
% equations
\newcommand{\eq}[2]{\begin{equation}  #2 \label{#1} \end{equation}}
\newcommand{\eql}[1]{\begin{equation} #1 \end{equation}}
\newcommand{\eqnotag}[1]{\begin{equation*}{#1}\end{equation*}}
%\newcommand{\eqkomma}[1]{\begin{equation}{#1}\komma\end{equation}}
%\newcommand{\eqpunkt}[1]{\begin{equation}{#1}\punkt\end{equation}}
%\newcommand{\eqdouble}[2]{\begin{equation}{#1}\komma\quad{#2}\punkt\end{equation}}
%\newcommand{\eqdoublek}[2]{\begin{equation}{#1}\komma\quad{#2}\komma\end{equation}}
%\newcommand{\eqtriple}[3]{\begin{equation}{#1}\komma\quad{#2}\komma\quad{#3}\punkt\end{equation}}
%\newcommand{\eqdtext}[3]{\begin{equation}{#1}\quad{\mbox{$\mbox{$\mathrm{#2}$}$}}\quad{#3}\end{equation}}
%\newcommand{\eqdtextdouble}[5]{\begin{equation}{#1}\quad{\mbox{$\mbox{$\mathrm{#2}$}$}}\quad{#3}\quad{\mbox{$\mbox{$\mathrm{#4}$}$}}\quad{#5}\end{equation}}
\newcommand{\eqdtextp}[3]{\begin{equation}{#1}\quad{\mbox{$\mbox{$\mathrm{#2}$}$}}\quad{#3}\punkt\end{equation}}
\newcommand{\eqdtriple}[3]{\begin{equation}{#1}\quad{#2}\quad{#3}\punkt\end{equation}}
\newcommand{\eqdoubleo}[2]{\begin{equation}{#1}\komma\quad{#2}\end{equation}}
\newcommand{\eqdoubleop}[2]{\begin{equation}{#1}\quad{#2}\punkt\end{equation}}
\newcommand{\eqdoubleok}[2]{\begin{equation}{#1}\quad{#2}\komma\end{equation}}
\newcommand{\eqdtripleo}[3]{\begin{equation}{#1}\komma\quad{#2}\komma\quad{#3}\end{equation}}
\newcommand{\eqdtripleoo}[3]{\begin{equation}{#1}\quad{#2}\quad{#3}\end{equation}}
\newcommand{\eqquatro}[4]{\begin{equation}{#1}\komma\quad{#2}\komma\quad{#3}\komma\quad{#4}\punkt\end{equation}}

% misc
\newcommand{\mat}[1]{\mbox{\boldmath$#1$}}
\newcommand{\tens}[1]{\mbox{\boldmath$#1$}}
\newcommand{\kmat}[1]{\mbox{\boldmath$\scriptstyle #1$}}
\renewcommand{\vec}[1]{\mbox{\boldmath$#1$}}
\newcommand{\symi}{^{\mathrm{sym}}}
\newcommand{\komma}{\mbox{$\mbox{$\, ,$}{}$}}
\newcommand{\kpomma}{\mbox{$\mbox{$\, ; \,$}{}$}}
\newcommand{\kkomma}{\mbox{$\mbox{$\, ,\quad$}{}$}}
\newcommand{\punkt}{\mbox{$\mbox{$\, .$}{}$}}
\newcommand{\scalar}[1]{\mbox{$\mbox{${#1}$}$}}
\newcommand{\kronecker}[2]{\mbox{$\mbox{$\delta_{#1#2\phantom{j}\!\!\!}$}$}}
\def\drunter#1#2{\mathop{#1}\limits_{#2}}
%\def\drueber#1#2{\mathop{#1}\limits^{\scriptscriptstyle #2}}
\def\drueber#1#2{\mathop{#1}\limits^{#2}}
\def\drueberunddrunter#1#2#3{\mathop{#1}\limits^{\scriptstyle
#2}_{\scriptstyle#3}}
\newcommand{\dole}[1]{_{\,\mathbf{#1}}}
\newcommand{\gore}[1]{^{\,\mathbf{#1}}}
\newcommand{\D}{\displaystyle}
\newcommand{\taui}{\tau^\mathrm{(i)}}
\newcommand{\disp}{\vec{\varphi}}
\newcommand{\isopotrate}{\dot{\mathcal{I}}_\mathrm{inc}^\mathrm{iso}}
\newcommand{\pot}{\mathcal{I}_{\mathrm{inc}}}
\newcommand{\Iinc}{\pot}
\newcommand{\potrate}{\dot{\mathcal{I}}_{\mathrm{inc}}}
\newcommand{\dlambda}{\Delta \lambda}
\newcommand{\Dint}{\mathcal{D}_{\mathrm{int}}}
\newcommand{\pvisco}{\alpha}
\newcommand{\bodyref}{{\mathcal{B}_0}}
\newcommand{\bodycur}{{\mathcal{B}_\mathrm{t}}}
\newcommand{\Lp}{{\boldsymbol{L}^\mathrm{p}}}
\newcommand{\Je}{{J^\mathrm{e}}}
\newcommand{\Jp}{{J^\mathrm{p}}}
\newcommand{\Pdisp}{\mathcal{P}_{\disp}}
\newcommand{\extforce}{{\boldsymbol{f}^\mathrm{ext}}}
\newcommand{\dt}{\Delta t}
\newcommand{\Gfb}{G^{(i)}_\mathrm{FB}}
\newcommand{\Gal}{G^{(i)}_\mathrm{al}}
\newcommand{\Gmin}{G^{(i)}_\mathrm{min}}
\newcommand{\sym}{^{\mathrm{sym}}}
\newcommand{\pl}{^{\mathrm{p}}}
\newcommand{\intr}{^{\mathrm{intr}}}
\newcommand{\glob}{^{\mathrm{glob}}}
\newcommand{\kk}{^{\mathrm{k}}}
\newcommand{\el}{^{\mathrm{e}}}
\newcommand{\ssi}{^{\mathrm{(i)}}}
\newcommand{\ssj}{^{\mathrm{(j)}}}
\newcommand{\nsys}{n_\mathrm{sys}}
\newcommand{\aset}{\mathbb{a}}
\newcommand{\F}{\tens{F}}
\newcommand{\Fp}{\tens{F}\pl}
\newcommand{\phip}{\varphi^\mathrm{p}}
\newcommand{\vecphip}{\vec{\varphi}^\mathrm{p}}
\newcommand{\identity}{\mat{1}}
\newcommand{\dIdlambda}{\frac{\partial \pot}{\partial \dlambda\ssi}}

%
% CP
%
\newcommand{\MdN}[1]{\vec{M}^{(#1)}\otimes\vec{N}^{(#1)}}
\newcommand{\schmid}{\tau}
%
% Mechanics
% ------------------
%\renewcommand{\vec}[1]{\fett{#1}}
%\newcommand{\tensvier}[1]{\mbox{$\mathbb{#1}$}}
\newcommand{\jacobi}{\mbox{$\mbox{${J}$}$}}
%Biblioteka
% ------------------
%\newcommand{\citeay}[1]{\citeauthor{#1} \citeyear{#1}}
% allgemeine Rechnenoperationen
% -----------------------------
\renewcommand{\ln}[1]{\mbox{$\mbox{$\mathrm{ln}\left({#1}\right)$}$}}
\renewcommand{\log}[1]{\mbox{$\mbox{$\mathrm{log}\left({#1}\right)$}$}}
\renewcommand{\sin}[1]{\mbox{$\mbox{$\mathrm{sin}\left({#1}\right)$}$}}
\renewcommand{\tan}[1]{\mbox{$\mbox{$\mathrm{tan}\left({#1}\right)$}$}}
\renewcommand{\cos}[1]{\mbox{$\mbox{$\mathrm{cos}\left({#1}\right)$}$}}
\renewcommand{\det}[1]{\mbox{$\mbox{$\mathrm{det}\left({#1}\right)$}$}}
\newcommand{\summe}[2]{\mbox{$\mbox{$\displaystyle\sum_{#1}^{#2}$}$}}
\newcommand{\bruch}[2]{\mbox{$\mbox{$\displaystyle\frac{#1}{#2}$}$}}
\newcommand{\totald}[1]{\mbox{$\mbox{$\mathrm{d}#1$}$}}
\newcommand{\total}[2]{\mbox{$\mbox{$\displaystyle\frac{\mathrm{d}#1}{\mathrm{d}#2}$}$}}
\newcommand{\derivs}[1]{\mbox{$\mbox{$#1'$}$}}
\newcommand{\derivsdr}[1]{\mbox{$\mbox{$#1''$}$}}
\newcommand{\partielld}[1]{\mbox{$\mbox{$\partiell#1$}$}}
\newcommand{\partiell}[2]{\mbox{$\mbox{$\displaystyle\frac{\partial#1}{\partial#2}$}$}}
\newcommand{\secondpartiell}[2]{\mbox{$\mbox{$\displaystyle\frac{\partial{}^2{#1}}{\partial{#2}^2}$}$}}
\newcommand{\secondpartiellver}[3]{\mbox{$\mbox{$\displaystyle\frac{\partial{}^2{#1}}{\partial{#2}\partial{#3}}$}$}}
\newcommand{\matrate}[1]{\mbox{$\mbox{$\mathbf{\dot{#1}}$}$}}
\newcommand{\matrrate}[1]{\mbox{$\mbox{$\mathbf{\ddot{#1}}$}$}}
\newcommand{\matrates}[1]{\mbox{$\mbox{$\dot{#1}$}$}}
\newcommand{\norm}[1]{\| {#1} \|}
\newcommand{\integral}[4]{\int \limits_{#1}^{#2} {#3} \, \mathrm{d} {#4} }
%
% Symbols
% -------------------------------------
\newcommand{\tensgreek}[1]{\mbox{$\mbox{\boldmath$#1$}$}}
\newcommand{\tensviera}[1]{\mbox{$\pmb{\mathbb{#1}}$}}
\newcommand{\tensrate}[1]{\mbox{$\dot{\mbox{$\mathbf{#1}$}}$}}
\newcommand{\tensgreekrate}[1]{\mbox{$\dot{\mbox{\boldmath$#1$}}$}}
\newcommand{\vectgreek}[1]{\mbox{$\mbox{\boldmath$#1$}$}}
\newcommand{\tensvier}[1]{\mbox{$\mathbb{#1}$}}
%
% 
% ---------------------------------------
\def\scal{\cdot}
\def\crossprod{\times}
\def\dyad{\otimes}
\newcommand{\transp}[1]{\mbox{$\mbox{${#1}\,\!^{\mathrm{T}\phantom{j}\!\!\!}_{\
        \phantom{j}\!\!\!}$}$}}
\newcommand{\transpi}[1]{\mbox{$\mbox{${#1}\,\!^{\mathrm{-T}\phantom{j}\!\!\!}_{\
        \phantom{j}\!\!\!}$}$}}
\newcommand{\negtransp}[1]{\mbox{$\mbox{${#1}\,\!^{-\mathrm{T}\phantom{j}\!\!\!}_{\ \phantom{j}\!\!\!}$}$}}
\newcommand{\inverse}[1]{\mbox{$\mbox{${#1}\,\!^{-1\phantom{j}\!\!\!}$}$}}
%
% Operators
% --------------------
\renewcommand{\det}{\mbox{$\mbox{$\mathrm{det}\,$}$}}
\renewcommand{\div}{\mbox{$\mbox{$\mathrm{div}$}$}}
%\newcommand{\dim}{\mbox{$\mbox{$\mathrm{dim}$}$}}
\newcommand{\inc}{\mbox{$\mbox{$\bigtriangleup$}$}}
\newcommand{\sign}{\mbox{$\mbox{$\mathrm{sign}$}$}}
\newcommand{\Div}{\mbox{$\mbox{$\mathrm{Div}$}$}}
\newcommand{\syml}[1]{\mbox{$\mbox{$\mathrm{sym\left({#1}\right)}$}$}}
\newcommand{\skw}[1]{\mbox{$\mbox{$\mathrm{skew\left({#1}\right)}$}$}}
\newcommand{\deriv}[1]{\mbox{$\mbox{$(#1)'$}$}}
\newcommand{\derivdr}[1]{\mbox{$\mbox{$(#1)''$}$}}
\newcommand{\Gradd}{\mbox{$\mbox{$\nabla_{\!0}$}$}}
\newcommand{\gradd}{\mbox{$\mbox{$\nabla$}$}}
\newcommand{\Grad}{\mbox{$\mbox{$\mathrm{GRAD}\,$}$}}
\DeclareMathOperator{\GRAD}{GRAD}
\DeclareMathOperator{\DIV}{DIV}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\EXP}{EXP}
\DeclareMathOperator*{\stat}{stat}
\DeclareMathOperator{\trace}{tr}
%
% Highlightcolor
\newcommand{\highlight}[1]{\textcolor{red}{#1}}
